Joint Channel and Weight Pruning for Model Acceleration on Moblie Devices

For practical deep neural network design on mobile devices, it is essential to consider the constraints incurred by the computational resources and the inference latency in various applications. Among deep network acceleration related approaches, pruning is a widely adopted practice to balance the computational resource consumption and the accuracy, where unimportant connections can be removed either channel-wisely or randomly with a minimal impact on model accuracy. The channel pruning instantly results in a significant latency reduction, while the random weight pruning is more flexible to balance the latency and accuracy. In this paper, we present a unified framework with Joint Channel pruning and Weight pruning (JCW), and achieves a better Pareto-frontier between the latency and accuracy than previous model compression approaches. To fully optimize the trade-off between the latency and accuracy, we develop a tailored multi-objective evolutionary algorithm in the JCW framework, which enables one single search to obtain the optimal candidate architectures for various deployment requirements. Extensive experiments demonstrate that the JCW achieves a better trade-off between the latency and accuracy against various state-of-the-art pruning methods on the ImageNet classification dataset. Our codes are available at https://github.com/jcw-anonymous/JCW.

==> tabels/joint-motivation.tex <==
\begin{table}[t]
    \centering
    %\scriptsize
    \setlength\tabcolsep{14pt}
    \begin{tabular}{l|ccc}
    \Xhline{2\arrayrulewidth}
         Method & Type & Latency & Accuracy \\
         \hline
         
                                Fast & Weight Pruning & 88.94 ms & 72.0\% \\
                              DMCP & Channel Pruning & 82.95 ms & 72.4\% \\
                             \hline
                             Fast & Weight Pruning & 35.89 ms & 65.2\% \\
                             DMCP & Channel Pruning & 33.50 ms & 62.7\% \\
    \Xhline{2\arrayrulewidth}         
    \end{tabular}
    \caption{Latency \& accuracy of MobileNetV2 models accelerated by fast sparse convolution~\cite{elsen2020sparsecov} and DMCP~\cite{guo2020dmcp}. The best acceleration strategy differs under various latency budgets.}
    \label{tab:joint-motivation}
\end{table}

==> tabels/joint-search-influence.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{l|ccc}
    % \toprule
    \Xhline{2\arrayrulewidth}
    % \hline
         Method & Latency & Accuracy \\
        %  \hline
        \Xhline{1.5\arrayrulewidth}
         \multirow{5}{*}{CWO} & 161.14 ms & 66.78\% \\
                                          ~ & 205.03 ms & 67.75\% \\
                                          ~ & 219.38 ms & 67.56\% \\
                                          ~ & 265.57 ms & 68.36\% \\
                                          ~ & 339.52 ms & 69.79\% \\
         \hline
         \multirow{4}{*}{WSO} & 161.72 ms & 68.45\% \\
                                            ~ & 196.82 ms & 69.54\% \\
                                            ~ & 200.50 ms & 69.57\% \\
                                            ~ & 220.07 ms & 70.09\% \\
        %  \hline
         \Xhline{1.5\arrayrulewidth}
         \multirow{4}{*}{JCW~(Ours)} & 160.37 ms & 69.16\% \\
                                   ~ & 193.65 ms & 69.70\% \\
                                   ~ & 196.44 ms & 69.90\% \\
                                   ~ & 223.73 ms & 70.19\% \\
        %  \hline
        \Xhline{2\arrayrulewidth}
        %  \bottomrule
    \end{tabular}
    \caption{Comparison of different variants of JCW. CWO~(Channel Width Only) denotes models with different searched number of channels. WSO~(Weight Sparsity Only) denotes only models with different searched layer-wise sparsity. The JCW with joint search of channel width and weight sparsity outperforms all the variants. The experiments are conducted with ResNet18 on ImageNet.}
    \label{tab:joint-search-influence}
\end{table}

==> tabels/separately.tex <==
\begin{table}[!bt]
    \centering
    \begin{tabular}{l|cc}
    \Xhline{2\arrayrulewidth}
         Search & Latency & Accuracy \\
         \hline
         \multirow{4}{*}{Separately} & 197.62 ms & 69.29\% \\
                                     & 221.65 ms & 69.58\% \\
                                     & 266.59 ms & 69.98\% \\
                                     & 305.78 ms & 70.20\% \\
        \hline
        \multirow{4}{*}{Jointly (OURS)} & 160.37 ms & 69.16\% \\
                                        & 193.65 ms & 69.70\% \\
                                        & 196.44 ms & 69.90\% \\
                                        & 223.73 ms & 70.13\% \\
        \Xhline{2\arrayrulewidth}
    \end{tabular}
    \caption{Influence of searching for channel pruning and weight pruning simultaneously. Separately means to first search for channel pruning, and then search for weight pruning. The experiments are conducted on Resnet18 on Imagenet.}
    \label{tab:separately-search}
\end{table}
